ImmunoFOMO: Are Language Models missing what oncologists see?

Language models (LMs) capabilities have grown with a fast pace over the past decade leading researchers in various disciplines, such as biomedical research, to increasingly explore the utility of LMs in their day-to-day applications. Domain specific language models have already been in use for biomedical natural language processing (NLP) applications. Recently however, the interest has grown towards medical language models and their understanding capabilities. In this paper, we investigate the medical conceptual grounding of various language models against expert clinicians for identification of hallmarks of immunotherapy in breast cancer abstracts. Our results show that pre-trained language models have potential to outperform large language models in identifying very specific (low-level) concepts.

==> Figures/alignment_reformatted.tex <==
\begin{figure*}[htbp]
    \centering

    % --- Row 1 ---
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.3\textwidth]{fig1.png}
        \hfill
        \includegraphics[width=0.3\textwidth]{fig2.png}
        \hfill
        \includegraphics[width=0.3\textwidth]{fig3.png}

        \captionof{figure}{Caption for the first row of images.}
    \end{minipage}

    \vspace{1cm}

    % --- Row 2 ---
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.3\textwidth]{fig4.png}
        \hfill
        \includegraphics[width=0.3\textwidth]{fig5.png}
        \hfill
        \includegraphics[width=0.3\textwidth]{fig6.png}

        \captionof{figure}{Caption for the second row of images.}
    \end{minipage}

    % --- Overall caption ---
    \caption{Overall caption for the 2x3 image grid, describing the entire figure.}
    \label{fig:overall_2x3}

\end{figure*}

==> Tables/hallu.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c ccc}
    \toprule
         & \textbf{Tier-I} & \textbf{Tier-II} & \textbf{Tier-III} \\
         \midrule
         PLMs&  -  & - & -\\
         LLMs& 0.004& 0.08 & 0.57\\
         \bottomrule
    \end{tabular}
    \caption{Hallucination percentage for language models.}
    \label{tab:hallu}
\end{table}
